Procedures as Programs: Hierarchical Control of Situated Agents through Natural Language

When humans conceive how to perform a particular task, they do so hierarchically: splitting higher-level tasks into smaller sub-tasks. However, in the literature on natural language (NL) command of situated agents, most works have treated the procedures to be executed as flat sequences of simple actions, or any hierarchies of procedures have been shallow at best. In this paper, we propose a formalism of procedures as programs, a powerful yet intuitive method of representing hierarchical procedural knowledge for agent command and control. We further propose a modeling paradigm of hierarchical modular networks, which consist of a planner and reactors that convert NL intents to predictions of executable programs and probe the environment for information necessary to complete the program execution. We instantiate this framework on the IQA and ALFRED datasets for NL instruction following. Our model outperforms reactive baselines by a large margin on both datasets. We also demonstrate that our framework is more data-efficient, and that it allows for fast iterative development.

==> cases.tex <==
\begin{table*}[t]\small
\centering
\begin{tabular}{ll}
\toprule
\textbf{Natural language instruction} & cook an egg with the microwave\\ 
\midrule
\textbf{Atomic action library \Aa} & 
\action{MoveAhead}, \action{RotateRight}, ...,  \\ 
& \action{Open} \object{object}, \action{Close} \object{object} \\
& \action{Put} \object{object} \object{receptacle}, \action{Pickup} \object{object} \object{receptacle},... \\
\midrule
\textbf{Case 1} (the egg is in the fridge) & \action{MoveAhead}, \action{MoveAhead}, \action{RotateRight}, ..., \\
& \action{Open} \object{fridge}, \action{Pickup} \object{egg} \object{fridge}, \action{Close} \object{fridge}, ..., \\
& \action{Open} \object{microwave}, \action{Put} \object{egg} \object{microwave} ... \\

\midrule
\textbf{Case 2} (the egg is in the countertop) &  \action{MoveAhead}, ..., \action{Pickup} \object{egg} \object{countertop}, ..., \action{Open} \object{microwave}, ... \\
\bottomrule
\end{tabular}
\caption{Two different atomic action sequences for the same natural language instruction. \action{action} represents atomic actions and \object{argument} represents the arguments and their concrete assignments. Note that the arguments should be realized as masks, we show the discrete symbols for simplicity. $\ldots$ indicates actions elided to save space. }
\label{tab:cases}
\end{table*}




==> pfunc_library.tex <==
\begin{figure}[htbp]
\begin{minted}{python}
def udp_close_if_needed(obj):
    reactor = get_reactor("check_obj_attr")
    attr = reactor(obj)
    if attr.is_openable and attr.is_open:
        atomic_close_object(obj)
def udp_postpare_recep(obj):
    reactor = get_reactor("check_obj_attr")
    attr = reactor(obj)
    if attr.is_openable and attr.is_open:
        atomic_close_object(obj)
def udp_pick_object(obj):
    reactor = get_reactor("find_obj_recep")
    udp_navigation(obj)
    recep = reactor(obj)
    udp_prepare_recep(recep)
    # this is for pickup laptop only
    udp_close_if_needed(obj)
    atomic_pick_object(obj)
    udp_postpare_recep(recep)
def udp_put_object(obj, dst):
    udp_navigation(dst)
    udp_prepare_recep(dst)
    atomic_put_object(obj, dst)
    udp_postpare_recep(dst)
def udp_clean_object(obj):
    # sink and faucet are global variables
    udp_pick_object(obj)
    udp_put_object(obj, sink)
    atomic_toggleon_object(faucet)
    atomic_toggleoff_object(faucet)
    udp_pick_object(obj)
def udp_slice_object(obj, tool_dst):
    # knife is a global variable
    udp_pick_object(knife)
    udp_navigation(obj)
    reactor = get_reactor("find_obj_recep")
    recep = reactor(obj)
    udp_prepare_recep(recep)
    atomic_slice_object(obj)
    udp_postpare_recep(recep)
    udp_put_object(tool, tool_dst)
def udp_pick_and_put_object(obj, dst):
    udp_pick_object(obj)
    udp_put_object(obj, dst)
def udp_cool_object(obj):
    # fridge is a global variable
    udp_pick_and_put_object(obj, fridge)
\end{minted}
\vspace{-0.7cm}
\caption{Procedural functions defined for ALFRED.}
\label{alfred_code_full}
\end{figure}
